Weights Shuffling for Improving DPSGD in Transformer-based Models

Differential Privacy (DP) mechanisms, especially in high-dimensional settings, often face the challenge of maintaining privacy without compromising the data utility. This work introduces an innovative shuffling mechanism in Differentially-Private Stochastic Gradient Descent (DPSGD) to enhance the utility of large models at the same privacy guarantee of the unshuffled case. Specifically, we reveal that random shuffling brings additional randomness to the trajectory of gradient descent while not impacting the model accuracy by the permutation invariance property -- the model can be equivalently computed in both forward and backward propagations under permutation. We show that permutation indeed improves the privacy guarantee of DPSGD in theory, but tracking the exact privacy loss on shuffled model is particularly challenging. Hence we exploit the approximation on sum of lognormal distributions to derive the condition for the shuffled DPSGD to meet the DP guarantee. Auditing results show that our condition offers a DP guarantee quite close to the audited privacy level, demonstrating our approach an effective estimation in practice. Experimental results have verified our theoretical derivation and illustrate that our mechanism improves the accuracy of DPSGD over the state-of-the-art baselines on a variety of models and tasks.

==> arxiv/outline.tex <==
% 验证sum of log-normal的近似情况，比较不同的方法近似情况
% 收集前面的结果，查漏补缺，多种dim情况的近似结果
% 图的方式进行呈现


% 验证shuffle不影响模型结果
% 通过shuffle的部署，验证模型的在shuffle前后结果一致
% 完成实验：
% 固定随机种子，shuffle与unshuffle的参数变换后完全一致
% 验证实验：VIT-CIFAR10和BERT-sst-2，完成表格，输出训练结束后的acc和loss
% [] 加上non-private的shuffle和unshuffle的验证
% [] VIT CIFAR10 shuffle和unshuffle
% [] BERT sst-2 shuffle和unshuffle

% 验证shuffled-DPSGD的acc能够提升
% 基于Attention-based architectures的实验
% [] VIT-CIFAR10, fixed ResNet, 
% [] BERT-sst-2, mnli, qnli, qqp
% [] roberta sst-2, mnli, qnli, qqp
% [] gpt-2 E2E, DART（nltk.translate.meteor_score)
% 形成一个大的实验结果表格
% 配上对应的文章Baseline（ghostclipping)  MixOpt （DPSGD）

% PRV accountant进行shuffle/ unshuffle的对比，在不同的eps和dim下，不同的sigma的结果
% 计算在相同的sigma，delta，和DPSGD的训练参数下的epsilon对比情况（图）
% 在训练情境下，给出shuffle和unshuffle的对比，绘制不同的图，代码不同的模型和shuffle的维度
% [] 在fix住conv层的情况下，用pretrain的模型，训练Wide ResNet50-2，对比shuffle和unshuffle，在不同epsilon的情况下，sigma的区别 训练参数量：51210
% [] 在pretrained Bert中，使用训练mnli的参数，对比shuffle和unshuffle，在不同epsilon的情况下，sigma的区别，参数量 ：110M
% [] 在pretrained GPT-2中使用训练e2e的参数，对比shuffle和unshuffle，在不同epsilon的情况下，sigma的区别，参数量：163M

% Aduting测试，在shuffled-DPSGD中，实际能满足的差分隐私大小
% 在VIT、BERT、roberta、gpt-2中，各选择一个数据集，做一个Aduting测试，尽量在设定单次噪声早小的情况下，测试shuffle/unshuffle的Empirical Epsilon 的对比
% [] 在VIT 训练CIFAR-10中进行aduting测试，测试shuffle/unshuffle的Empirical Epsilon 的对比

% 检测shuffle带来的overhead有多大

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% 修改意见
% improving privacy of DPSGD with shuffling on Large Model

% 根据这个可以提出，shuffled-DPSGD
% 介绍这个思想，

% 第三段开始需要突出high-dimension的挑战的困难。
% 并且指出前面工作的不足之处，例如：降维，调参工作的局限性

% 在intro部分介绍motivation，

% 技术难点，high-dim，sum of log normal， mixture Gaussian，提升的具体的数值，approximate。做aduting满足了eps，delta-DP， highlight 挑战

% permutation invariance of large models. 规范一下large model的种类，
% shuffle
% 在主流的模型上的适用性，

% 通过prv的composition可以提升DPSGD的accountant？

% 3 challenge 加粗，
% 解决high dim，用shuffle机制，对应Sec 4.1 4.2 Method, 对应第二、三个RQ，shuffle不改变模型结果，shuffle机制能够提升模型ACC
% 用近似保证eps，delta-DP的充要条件，对应Sec 4.3，对应第一个RQ，验证不同的近似方法
% 给shuffled-DPSGD进行privacy accountant，对应Sec 5.1 5.2，对应第四个RQ，验证shuffled-DPSGD的隐私保证
% Auditing的验证, 对应Sec 5.3，对应第五个RQ，验证shuffled-DPSGD的eps的实际大小
% 提升的具体的数值，适用的模型的范围具体
% highlights contribution

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 1.15的修改意见
% intro中，motivation一方面是对噪声的影响，另一方面是对shuffle mechanism的design，如何在shuffle的过程中，保证结果的不变性。
% 3.2主要介绍模型结构，invariance放在后面
% Shuffle permutation放在related work里面，前面工作的介绍，和本文的不同之处，然后是def 2放在第四章
% 在第四章，明确写解决challengeX，需要先介绍motivation，介绍为什么需要引入shuffle，然后是引入shuffle的担心，引用前文的工作，过度到对shuffle invariance的介绍，对模型本身的影响，P3介绍
% 尽管只有两个层，看起来非常局限，起到了非常大的作用，并且参数量占了很大的比重
% l2 放前面，def 3和后面的公式加入标点符号
% 在4.1靠后的位置定义好P_s，这个操作是对模型里面的linear层和Transformer层进行的shuffle，对与剩下的层是进行的fix，def
% 在4.2统一shuffle的符号P_s

% 解释在实际的shuffle中是矩阵，但是在分析中我们统一用向量进行分析，解释shuffle的一致性
% 在prelim里面介绍一下，sum of lognormal的F-W方法

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Introduction Outlines

1. Background and Motivation: Highlights the risk of information leakage in trained neural networks and introduces Differential Privacy (DP) as a solution to quantify and limit this leakage.

2. Challenges in DPSGD: Discusses the significant accuracy loss in conventional Differentially Private Stochastic Gradient Descent (DPSGD) due to noise perturbation, especially in high-dimensional data.

3. High-Dimensional DPSGD Challenges: Addresses the challenge of managing large noise perturbations in high-dimensional DPSGD and explores low-dimensional gradient approximations as a potential solution.

4. Motivation of Shuffled-DPSGD as a Solution: Introduces shuffled-DPSGD to enhance DP privacy in high-dimensional settings, focusing on reducing noise perturbation while maintaining model performance.

5. Challenges of Privacy Accounting in Shuffled-DPSGD: Discusses the challenge of calculating differential privacy metrics for shuffled Gaussian mechanisms and the development of a new privacy accountant.

6. Contributions of the Work: Summarizes the paper's contributions, including the novel shuffled-DPSGD approach, proving its differential privacy conditions, and validating its effectiveness through experiments.

7. Paper Organization: Outlines the structure of the paper, including sections on related work, Preliminaries, methodology, algorithm, experimental results, and conclusions.

Experiments Outlines

Sec 6. Introduction to Experiments: Introduces the experimental section, focusing on the research question and experimental design.

Sec 6.1 Experimental Setup: Describes the experimental settings, including dataset and model introductions, and specific experimental configurations.

Sec 6.1.1 Tasks, Models, and Datasets: Details the tasks and datasets used in the experiments, covering classification tasks in computer vision (CV) and natural language processing (NLP), as well as generation tasks in NLP.

Sec 6.1.2 Metric: Explains the evaluation metrics used for the experiments.

Sec 6.1.3 Baseline: Introduces advanced works in DPSGD as baselines for comparison, including Ghost clipping, MixOpt.

Sec 6.1.4 Implementation Details: Discusses the practical aspects of implementing the experiments, including settings for PRV accountant and shuffled-DPSGD.

Sec 6.1.5 Shuffle Implementation: Describes the actual implementation of the shuffle mechanism and compares different methods for efficiency.

Sec 6.2 Experiments of Parameters Permutation Invariance: Verifies the Parameters Permutation Invariance of the shuffle mechanism through experiments on different models.

Sec 6.3 Experiments Privacy Accountant of Shuffled-DPSGD: Conducts numerical experiments and analysis on the privacy accountant of shuffled-DPSGD, comparing different approximation methods.

Sec 6.4 Results of Shuffled-DPSGD: Presents the results of shuffled-DPSGD in large model training for CV classification, NLP classification, and NLP generation tasks, comparing with baseline models.

Sec 6.5 Auditing the Privacy of Shuffled-DPSGD: Verifies the correctness of the privacy accountant calculation for shuffled-DPSGD through auditing methods.

Sec 6.6 Overhead of Shuffled-DPSGD: Analyzes the additional computational overhead required by shuffled-DPSGD, focusing on the shuffle operation's time cost.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%修改意见 1.30
1、 表一没有任务
2、 一般实验section开头列下research question会比较清晰,然后实验各个小节要表明是回答哪个RQ
3、 一般不展示代码 可放附录
4、 baseline里需要介绍下Ghost clipping和mixopt用的是什么基本机制 以及什么accountant
5、 表1还补充下 可shuffle的参数占总的参数的比例
6、 fig2想要突出参数量的影响的话 把shuffled 参数量标在模型名称后面
7、 而且没有对实验现象的分析解释 比方说对于不同的epsilon 为什么sigma是近乎一样的？从算法层面分析是什么原因
8、 tab3和fig2往前移一页、和相关文字放一起
9、 tab4的epsilon太少了至少再跑2个epsilon 往小一个往大一个
10、 表4、5要和对应的文字放在一页上

% 修改意见
% improving privacy of DPSGD with shuffling on Large Model

% 根据这个可以提出，shuffled-DPSGD
% 介绍这个思想，

% 第三段开始需要突出high-dimension的挑战的困难。
% 并且指出前面工作的不足之处，例如：降维，调参工作的局限性

% 在intro部分介绍motivation，

% 技术难点，high-dim，sum of log normal， mixture Gaussian，提升的具体的数值，approximate。做aduting满足了eps，delta-DP， highlight 挑战

% permutation invariance of large models. 规范一下large model的种类，
% shuffle
% 在主流的模型上的适用性，

% 通过prv的composition可以提升DPSGD的accountant？

% 3 challenge 加粗，
% 解决high dim，用shuffle机制，对应Sec 4.1 4.2 Method, 对应第二、三个RQ，shuffle不改变模型结果，shuffle机制能够提升模型ACC
% 用近似保证eps，delta-DP的充要条件，对应Sec 4.3，对应第一个RQ，验证不同的近似方法
% 给shuffled-DPSGD进行privacy accountant，对应Sec 5.1 5.2，对应第四个RQ，验证shuffled-DPSGD的隐私保证
% Auditing的验证, 对应Sec 5.3，对应第五个RQ，验证shuffled-DPSGD的eps的实际大小
% 提升的具体的数值，适用的模型的范围具体
% highlights contribution

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 1.15的修改意见
% intro中，motivation一方面是对噪声的影响，另一方面是对shuffle mechanism的design，如何在shuffle的过程中，保证结果的不变性。
% 3.2主要介绍模型结构，invariance放在后面
% Shuffle permutation放在related work里面，前面工作的介绍，和本文的不同之处，然后是def 2放在第四章
% 在第四章，明确写解决challengeX，需要先介绍motivation，介绍为什么需要引入shuffle，然后是引入shuffle的担心，引用前文的工作，过度到对shuffle invariance的介绍，对模型本身的影响，P3介绍
% 尽管只有两个层，看起来非常局限，起到了非常大的作用，并且参数量占了很大的比重
% l2 放前面，def 3和后面的公式加入标点符号
% 在4.1靠后的位置定义好P_s，这个操作是对模型里面的linear层和Transformer层进行的shuffle，对与剩下的层是进行的fix，def
% 在4.2统一shuffle的符号P_s

% 解释在实际的shuffle中是矩阵，但是在分析中我们统一用向量进行分析，解释shuffle的一致性
% 在prelim里面介绍一下，sum of lognormal的F-W方法

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

/**
 * Title: Improving Privacy of DPSGD with Shuffling on Large Model
 * 
 * Introduction:
 * This documentation comment introduces the concept of shuffled-DPSGD and highlights the challenges in dealing with high-dimensional data. It also mentions the limitations of previous works, such as dimensionality reduction and the limitations of parameter tuning.
 * 
 * Motivation:
 * The motivation behind this work is explained in the introduction section.
 * 
 * Technical Challenges:
 * The technical challenges include dealing with high-dimensional data, handling the sum of log-normal and mixture Gaussian distributions, achieving specific numerical improvements, and approximations. The auditing process ensures the satisfaction of epsilon-delta differential privacy and highlights the challenges faced.
 * 
 * Permutation Invariance of Large Models:
 * This section discusses the different types of large models and emphasizes the importance of shuffling in achieving permutation invariance. It also mentions the applicability of shuffled-DPSGD on mainstream models.
 * 
 * Improving DPSGD Accountant through PRV Composition:
 * This section explains how the privacy accounting of DPSGD can be enhanced through PRV composition.
 */

